RL4ReAl: Reinforcement Learning for Register Allocation

We aim to automate decades of research and experience in register allocation, leveraging machine learning. We tackle this problem by embedding a multi-agent reinforcement learning algorithm within LLVM, training it with the state of the art techniques. We formalize the constraints that precisely define the problem for a given instruction-set architecture, while ensuring that the generated code preserves semantic correctness. We also develop a gRPC based framework providing a modular and efficient compiler interface for training and inference. Our approach is architecture independent: we show experimental results targeting Intel x86 and ARM AArch64. Our results match or out-perform the heavily tuned, production-grade register allocators of LLVM.

==> table-runtimes.tex <==

\definecolor{ygreen}{HTML}{d6e39d}
\definecolor{sgreen}{HTML}{bee69c}
\definecolor{arylideyellow}{rgb}{0.91, 0.84, 0.42}
\definecolor{buff}{rgb}{0.94, 0.86, 0.51}
\definecolor{citrine}{rgb}{0.89, 0.82, 0.04}
\newcommand{\first}[1][]{\cellcolor{sgreen}}
\newcommand{\second}[1][]{\cellcolor{yellow}}


\begin{table}[h!tb]
\small
\centering
\caption{Improvement in runtimes (s) on x86 over \rabasic{} allocator. 
\colorbox{sgreen}{Highest} and \colorbox{yellow}{Second highest} improvements are highlighted.}
\label{tab:x86-runtime}
\begin{tabular}{lrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Benchmarks}}} &
  \multicolumn{1}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Runtime\\ \rabasic\end{tabular}}}} &
  \multicolumn{4}{c}{\textbf{Difference from \rabasic (\rabasic - x)}} \\
\cmidrule(lr){3-6}
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\multirow{2}{*}{\rapbqp}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\ragreedy}} &
  \multicolumn{2}{c}{\textbf{\toolname{}}} \\
\cmidrule(lr){5-6}
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{L}} &
  \multicolumn{1}{c}{\textbf{G}} \\
\midrule
401.bzip2              & 360.6       & -7.3  & \second 7.5   & -1.1  & \first 10.8  \\
429.mcf                & 233.8       & \second 1.4   & -2.9  & \first 2.7   & -3.6  \\
445.gobmk              & 322.3       & -3.3  & \first 6.4   & \second 2.4   & 1.7   \\
456.hmmer              & 284.3       & 1.8   & \first 6.1   & \second 5.0   & -37.6 \\
462.libquantum         & \first 256.4       & -10.1 & \second -1.1  & -2.2  & -6.7  \\
471.omnetpp            & 305.7       & \second 0.7   & \second 0.4   & \first 1.2   & \first 1.2   \\
433.milc               &\first 349.1       & -16.6 & \first 0.1   & -13.8 & \second -7.0  \\
470.lbm                & 184.0       & -7.9  & \first 3.0   & \second 2.3   & 1.4   \\
482.sphinx3            & 366.0       & -37.5 & \first 1.6   & -3.1  & \second -2.7  \\
\midrule
505.mcf\_r             & 344.9       & \second 4.5   & -1.6  & \first 8.6   & -4.7  \\
520.omnetpp\_r         & 475.7       & \first 6.4   & \first 6.4   & \second 2.4   & \second 2.8   \\
525.x264\_r            & 244.1       & \first 1.8   & \first 1.3   & -5.8  & -1.5  \\
531.deepsjeng\_r       & 299.9       & 4.6   & \first 16.0  & 9.9   & \second 12.8  \\
541.leela\_r           & 439.5       & 1.6   & \first 7.1   & 0.4   & \second 1.9   \\
557.xz\_r              & 371.5       & -0.6  & \second 11.9  & \first 12.1  & -8.5  \\
508.namd\_r            & 236.5       & 2.5   & \first 23.5  & 9.1   & \first 23.8  \\
519.lbm\_r             & 261.8       & 1.4   & \first 57.7  & \second 50.9  & \first 58.1  \\
538.imagick\_r         & 479.3       & -16.9 & \second 115.5 & \first 118.8 & \first 118.4 \\
544.nab\_r             & 417.5       & 5.8   & \second 132.1 & \second 131.3 & \first 134.4 \\
\midrule
\multicolumn{2}{r}{\textbf{Average}} & -3.6  & 20.6  & 17.4  & 15.5 \\
\bottomrule
\end{tabular}
\end{table}






\begin{table}[tb]
\caption{Improvement in runtimes (s) on AArch64 over \rabasic allocator. 
\colorbox{sgreen}{Highest} and \colorbox{yellow}{Second highest} improvements are highlighted.}
\label{tab:aarch64-runtime}
\small
\begin{tabular}{lrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Benchmarks}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Runtime\\ \rabasic\end{tabular}}}} &
  \multicolumn{3}{c}{\textbf{Difference from \rabasic (\rabasic - x)}} \\
  \cmidrule(lr){3-5} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\rapbqp}}} &
  \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\ragreedy}}} &
  \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\toolname{}}}} \\
%   \cmidrule(lr){5-6}
% \multicolumn{1}{c}{} &
%   \multicolumn{1}{c}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{c}{\textbf{G + TL}} &
%   \multicolumn{1}{c}{\textbf{G}} \\
\midrule
401.bzip2 &  1366.9 &   -41.1 &   \first 15.6  & \second 12.8 \\
429.mcf &   \second 1320.5 &   -12.7 &   -7.5 & \first 1.6\\
445.gobmk &   992.8 &    \second 15.6 &  \first 26.1  &  \second 14.5 \\
462.libquantum &   1627.6 &   -8.7 &   \second 4.5  & \first 9.6\\

433.milc &   1251.1 &  \second 59.2 &   \first 70.9  &  45.4\\
444.namd &   855.3 &   2.7 &   \first 21.8  &  \second 18.8\\
470.lbm &   1604.3 &   \second -6.4 &   -16.6  & \first 16\\
\midrule
505.mcf\_r & 1535.1 & \first 25.9 & \second 1.9 & -12.8\\
508.namd\_r & 845 & 0.4 & \second 34.5 & \first 40.1 \\
523.xalancbmk\_r &   979.1 &   \first 8.1 &   -3.4  & \second 4.4 \\
531.deepsjeng\_r &   777.2 &   \second 10.0 &   \first 30.5 & 4.5\\
541.leela\_r &   \first 1067.9 & \second -11.3 &   \first -0.1 & -19.5 \\
557.xz\_r &   1163.2 &   \second 3.7 &   \first 22.2 & \first 21.3\\
519.lbm\_r &   1657 &   \first 50.9 &   -1.6  & \second 39.8\\
538.imagick\_r &   1244.5 &   -3.9 &   \first 75.8 & \second 65.6\\
544.nab\_r &   \second 1170.7 &   -7.7 &   \first 31.5  &  \first 32.4\\
  \midrule
\multicolumn{2}{r}{\textbf{Average}} &   5.3 & 19.1 & 18.4\\
 \bottomrule

 \vspace{-1.0cm}
\end{tabular}
\end{table}
